ORMA: Optimization-based Monocular 4D Reconstruction of Articulated Animals

Recovering articulated 4D representations of animals from monocular videos remains challenging due to the large diversity of quadruped morphologies and lack of animal 4D supervision data. Existing learning-based reconstruction methods operate on individual images and rely on synthetic or model-fitted 3D supervision, which inherits the constraints of strong parametric priors and limits generalization to out-of-distribution species. When applied to out-of-distribution animals, they often recover a plausible pose while producing inaccurate geometry because the underlying shape model cannot faithfully represent the observed instance. We present ORMA, a training-free reconstruction framework that decouples articulation from shape, using the predicted pose as reference for optimization while leveraging generative 3D priors for accurate shape reconstruction. Given a reference image, we reconstruct the animal geometry and register it to the parametric model SMAL+, yielding an articulated shape adapted to the observed instance. We then combine per-frame articulated pose estimates with globally consistent camera poses to recover animal motion in a shared world coordinate frame, and further refine the reconstruction using self-supervised DINO correspondences and temporal consistency. To enable quantitative evaluation, we introduce PAW4D, a synthetic multi-species benchmark with ground-truth 3D geometry and camera motion. Experiments on PAW4D, PFERD, and challenging in-the-wild videos demonstrate that ORMA improves reconstruction accuracy while recovering globally consistend animal motion across diverse quadruped species.

==> sections/03_Background.tex <==
\subsection{SMAL}
\label{sec:SMAL}
The SMAL model \cite{Zuffi:CVPR:2017} follows the formulation of SMPL \cite{SMPL:2015} and represents animal shape and pose using a deformable mesh model. The model is defined by a triangular template mesh $\mathbf{v}_t$ with $n_V$ vertices, a linear shape space represented by a matrix $B \in \mathbb{R}^{3n_V \times n_B}$ containing $n_B$ shape basis vectors, a joint regressor $J_r$ that maps mesh vertices to a set of $n_J$ skeletal joint locations, and a skinning weight matrix $W$.
Given shape parameters $\beta \in \mathbb{R}^{n_B}$ and pose parameters $\theta$, a quadruped mesh is generated in two stages. First, the template mesh is deformed in the learned shape space to produce an intrinsic (rest) shape $\mathbf{v}_s$. Then, articulated pose deformations are applied using Linear Blend Skinning (LBS) to rotate the body parts according to the specified pose parameters:

\begin{eqnarray}
\textbf{v}_{s} & = & \textbf{v}_{t} + B \beta^T \nonumber \\
\textbf{v} & = & LBS(\textbf{v}_{s}, \theta; W, J_r). 
\label{eq:model}
\end{eqnarray}

\subsection{Animer/megasam}
\label{sec:NF}
AniMer \cite{lyu2025animer} tackles multi-species animal pose and shape estimation by directly regressing SMAL parameters from a single RGB image. It uses a Vision Transformer (ViT) encoder to extract image patch tokens together with a learnable class token, and feeds these features into a transformer decoder and MLP regression heads that predict SMAL pose and shape parameters (and camera parameters for projection).\\
MegaSaM \cite{li2025megasam} is a learning-augmented monocular SLAM/SfM pipeline designed for captured videos that contain scene dynamics. Building on a differentiable bundle-adjustment (BA) formulation, it predicts dense frame-to-frame correspondences and their uncertainties and then jointly optimizes camera parameters and per-frame depth over the sequence. To remain robust in dynamic scenes, MegaSaM learns a motion probability map and uses it to downweight pixels likely belonging to moving content during BA.

 


==> sections/04_Method.tex <==
\section{Method}

\mypar{Notation}
We will refer to $\mathcal{M}=S(\shape,\pose,\trasl,\grot)$ as the SMAL model instance we are optimising, where \colorbox{yellow}{$\beta \in \mathbb{R}^{41} $} are the shape parameters, $\theta \in \mathbb{R}^{3(J-1)}$ are the pose parameters in axis-angle representation, where \colorbox{yellow}{$J=35$} is the number of body joints, $\trasl \in \mathbb{R}^{3}$ is the global translation and $\grot \in SO(3)$ the global rotation.

For brevity, in the following we simply write $S$ and omit its parametrisation. 
% We will also denote $S_{H3D}$ SMAL where the $\beta$ are fixed by the registration to Hunyan.
The input to our method is a video $\mathbf{F} \in \mathbb{R}^{H \times W \times 3 \times N}$
composed of $N$ frames $\image{i} \in \mathbb{R}^{H \times W \times 3}$ of height $H$ and
width $W$.
We denote the binary foreground mask of the animal in frame $\image{i}$, obtained by
SAM~\cite{SAM}, as $M(\image{i}) \in \{0,1\}^{H \times W}$.
We define a differentiable image projector
\begin{equation}
    \pi(\,\cdot \mid C) \;:=\; \mathcal{M} \;\mapsto\; I_C^{\mathcal{M}} \in \mathbb{R}^{H \times W},
\end{equation}
that produces a rendered image $I_C^{\mathcal{M}}$ for a triangular mesh $\mathcal{M}$
observed by camera $C$.  In the following, when the camera $C$ is clear from the context, we will just write to $\pi(\,\cdot\,)$ for compactness.

% ---------------------------------------------------------------
\mypar{Initialisation: AniMer{+} and MegaSaM}
To bootstrap our optimisation, we first obtain a rough per-frame estimate of the animal
shape, pose, and camera parameters from AniMer{+}~\cite{AniMer}.  Since AniMer{+}
operates at the frame level its predictions may exhibit significant temporal
inconsistencies, as we demonstrate in the experimental section.
We then process the full video with MegaSaM~\cite{MegaSAM} to obtain accurate
camera-pose estimates and with SAM~\cite{SAM} to extract animal masks for every frame.



% ---------------------------------------------------------------
\subsection{ORMA: Optimization-based Monocular 4D Reconstruction of Articulated Animals}
\label{sec:orma}
% ---------------------------------------------------------------
\mypar{Accurate 3D Shape recovery}
Our goal is to obtain an accurate 3D shape of the target animal.
AniMer{+} predictions rely solely on SMAL statistics, which may not adequately capture
the morphology of a specific species, breed or individual.
We therefore take the first frame of the video and process it with
Hunyuan3D~\cite{zhao2025hunyuan3d20}, a generalist generative reconstruction backbone, which gives us a 3D textured mesh.
We then optimise the $S$ shape, pose, global rotation and translation parameters to register it to the Hunyuan3D output.
Concretely, we first globally align the AniMer{+} prediction with the Hunyuan3D reconstruction
using multi-start ICP, avoiding poor local minima (\eg, head aligned with the tail).
We then perform a standard registration via Chamfer optimisation with local displacements and ARAP
regularisation~\cite{ARAP}.
Full details of this step are given in the Supplementary Material.

After the initialisation step, the animal shape is fixed and no longer expressed in the SMAL shape space, but as the computed registration to the Hunyuan3D output, in the SMAL model topology. We refer to such registration as $S_{H3D}$.
In the following, we describe the losses used to recover the pose $\pose$, global
rotation $\grot$, and world-space translation $\trasl$ for every frame.

% ---------------------------------------------------------------
\mypar{Total Loss}
Our optimisation minimises a combination of appearance, depth, semantic, and
regularisation terms:
\begin{equation}
\label{eq:total}
    L_{\text{total}}(\pose,\trasl,\grot)
    = L_{\text{app}} + w_d L_{\text{depth}} + w_D L_{\text{DINO}}
      + w_p L_{\text{pose}} + w_vL_{\text{vert}}.
\end{equation}
Where $w_\star$ terms denote weights we tune on the validation set.
At every frame, the parameters are initialized from the previous frame, since we empirically found that this is better than starting from the AniMer prediction. Though we still compute AniMer poses for all frames and use them in our regularization terms, as we explain at the end of this section.


% ---------------------------------------------------------------
\mypar{2D Geometric Loss}
The 2D geometric loss encourages the projected template to align with the 2D observations
in the current frame $\image{i}$ and is composed of three terms:
\begin{equation}
\label{eq:app}
    L_{\text{app}} = w_dL_{\text{dice}} + w_pL_{\text{per}} + w_bL_{\text{bound}}.
\end{equation}
The first term is a Dice loss that aligns the silhouette of the projected template with the SAM mask:
\begin{equation}
    L_{\text{dice}}
    = 1 - \frac{2\,\bigl|\pi(S \mid C_i) \cap M(\image{i})\bigr|}
               {\bigl|\pi(S \mid C_i)\bigr| + \bigl|M(\image{i})\bigr|}.
\end{equation}
During our ablation study, we noticed that this loss is insufficient to achieve good alignment with the observed silhouette. Likely, the gradient does not provide enough signal on the boundary, leading to local minima. To reinforce the supervision, we therefore add two complementary boundary terms. \SZ{Questa può essere una technical novelty o è presente in altri lavori? Da mettere nell'ablation.}
The first enforces that the projected contour and the mask contour have the same
arc-length:
\begin{equation}
    L_{\text{per}}
    = \bigl\|
        \mathcal{L}\!\left(\partial\pi(S \mid C_i)\right)
        - \mathcal{L}\!\left(\partial M(\image{i})\right)
      \bigr\|,
\end{equation}
where $\partial(\cdot)$ denotes the boundary-extraction operator and
$\mathcal{L}(\cdot)$ the arc-length of a contour.
The second penalises the pixelwise difference between the soft boundary map of the
projected template and that of the mask.
Let $\mathcal{B}(\cdot) \in [0,1]^{H \times W}$ denote the soft boundary map of its
argument, where a value of $1$ indicates a boundary pixel and $0$ indicates a
non-boundary pixel.
Then:
\begin{equation}
    L_{\text{bound}}
    =\|
        \mathcal{B}\!\left(\pi(S \mid C_i)\right) -
        \mathcal{B}\!\left(M(\image{i})\right)\|_1
      .
\end{equation}
where $\mathcal{B}_S = \partial\pi(S \mid C_i)$ and
$\mathcal{B}_M = \partial M(\image{i})$ are the sets of boundary pixels for the
projected template and the mask, respectively.

% ---------------------------------------------------------------
\mypar{Depth Loss}
MegaSaM provides a reliable dense depth estimate for every frame, which we exploit
to add metric geometric supervision.
Let $D(\image{i}) \in \mathbb{R}^{H \times W}$ denote the depth map estimated by
MegaSaM for frame $\image{i}$, and $D(\pi(S \mid C_i)) \in \mathbb{R}^{H \times W}$
the depth buffer rendered from the current template. \SZ{Qui non ho capito il problema della scala nel video reale, il confronto è sempre diretto o dipendente dal video?}
We define:
\begin{equation}
    L_{\text{depth}}
    = \mathrm{MSE}\!\left(D\!\left(\pi(S \mid C_i)\right),\; D(\image{i})\right).
\end{equation}

% ---------------------------------------------------------------
\mypar{Semantic Loss}
The losses above can still admit local minima, \eg, limbs swapped from left to right. Animal Avatar \cite{dummy} solve this relying on Continuous Surface Embeddings, which we regard as sub-optimal since \RM{Spiegare perché quello che facciamo noi é meglio} \FP{Mostrare CSE Embeddings cs DINO}.
We therefore augment the optimisation with dense semantic guidance from DINO
features~\cite{DINO}. 
\SZ{Qui è importante capire se ciò che usiamo ha degli elementi di novità rispetto a previous work.}


\emph{Feature baking.}
We render $S_{H3D}$ 
%, the Hunyuan3D reconstruction obtained in during the $\shape$ optimization,
%\SZ{Penso che la mesh la dobbiamo "nominare" quando descriviamo la registrazione, e poi usiamo il simbolo da lì in avanti. Potrebbe essere una cosa tipo $S_{H3D}$.} 
from $V$ viewpoints
and extract a DINO feature map $\Phi_v \in \mathbb{R}^{H' \times W' \times d}$ for each
view $v$. Since DINO output features at $48 \times 48 $ resolution, we upscale them using AnyUp \cite{anyup}.
%\FP{Mi sono dimenticato di specificare che ho usato un modello chiamato AnyUp per upscalare le dino features, perchè di per se da un'immagine 256x256 dino restituisce delle feature di 48x48xDINODIM}.
We \colorbox{yellow}{project} \SZ{backproject?} these features onto the mesh vertices, and for the vertices visible in multiple
views we average the projected features:
\begin{equation}
    \mathbf{f}_u
    = \frac{1}{\bigl|\mathcal{V}(u)\bigr|}
      \sum_{v\,\in\,\mathcal{V}(u)} \Phi_v(u),
\end{equation}
where $\mathcal{V}(u)$ is the set of views in which vertex $u$ is visible and
$\Phi_v(u)$ is the feature projected onto vertex $u$ from view $v$. \SZ{Questa equazione si può eliminare perchè non descriviamo cose più complesse, tipo come determinare la visibilità dei vertici, o in cosa consiste la proiezione, però poi scriviamo in modo esplicito l'operazione di media. Si può scrivere ulteriori dettagli nel Supp Mat. se non c'è spazio.}
We refer to the mesh decorated by these per-vertex features $\{\mathbf{f}_u\}$ as
$\hat{S}$. 

\emph{Per-frame semantic correspondences.}
Given the decorated mesh $\hat{S_{H3D}}$, we render its feature map onto the image plane
of camera $C_i$, obtaining
$\Pi_i \in \mathbb{R}^{H' \times W' \times d}$,
where $\Pi_i^{\,j}$ is the feature vector at pixel $j$ of the rendered feature image.
We also extract a DINO feature map
$\tilde{F}_i \in \mathbb{R}^{H' \times W' \times d}$
directly from the video frame $\image{i}$.

\SZ{Questa sotto potrebbe essere la technical novelty. Penso che possiamo dire che altri metodi usano il matching tra le dino feature maps, ma questo può comportare di essere intrappolati in un minimo locale, mentre definire le corrispondenze supera il problema (vedo che lo hai anche scritto dopo).}
For each pixel $j$ inside the projected mask $\pi(M(\image{i}) \mid C_i)$ we define a
nearest-neighbour correspondence into the target feature map:
\begin{equation}
    \sigma_j
    \;:=\;
    \arg\min_{k \,\in\, \mathcal{P}_i}
    \bigl\|\Pi_i^{\,j} - \tilde{F}_i^{\,k}\bigr\|_2,
    \label{eq:correspondence}
\end{equation}
where $\mathcal{P}_i$ is the set of all valid (foreground) pixel indices in frame $i$. \SZ{L'equazione così secondo me non funziona perchè è la differenza tra una posizione una feature}. \RM{avevo sbagliato qui sotto la definizione di $\Pi_i^j$, ma l'equazione dovrebbe essere ok: è la differenza tra le feature del j-esimo pixel dell'immagine renderizzata e il k-esimo pixel del frame del video, e salviamo la posizione argmin in $\sigma_j$}
\SZ{Ok, questa formulazione è simile alla loss in Animal Avatar, giusto? (Eq. 6 di animal avatar). In questo caso dobbiamo mettere il riferimento e non è una technical novelty.}
The index $\sigma_j$ identifies, for every rendered feature pixel $j$, the
semantically closest pixel in the observed frame.
% Because $\sigma_j$ is computed via a hard $\arg\min$ it is treated as a \emph{fixed}
% index during the backward pass (\ie, we stop gradients through the correspondence
% assignment and differentiate only through the feature positions
% $\Pi_i^{\,j}$~\cite{PatchMatch}).
Using the correspondences from \cref{eq:correspondence}, we penalise the spatial
misalignment between the current template projection and the observed frame:
\begin{equation}
    L_{\text{DINO}}
    = \frac{1}{|\mathcal{P}_i|}
      \sum_{j \,\in\, \mathcal{P}_i}
      \bigl\|\Pi_i^{\,j} - \tilde{F}_i^{\,\sigma_j}\bigr\|_2^2.
    \label{eq:dino_loss}
\end{equation}
Intuitively, \cref{eq:dino_loss} pulls each rendered feature pixel towards the
semantically matching location in the target image, providing a long-range gradient
signal that complements the silhouette and depth losses.

% ---------------------------------------------------------------
\mypar{Regularisation Losses}
While the Animer pose is not always accurate, it provides a fair initialization to our process and we avoid too dramatic variations from it:
\begin{equation}
    L_{\text{pose}}
    = MSE(\pose, \pose_{animer}),
\end{equation}

\SZ{Qui o prima dobbiamo dire qual'è la nostra rappresentazione delle rotazioni. Poi questo loss è applicato in modo differente in base alla presenza o meno della soluzione di AniMer+, giusot?}
We also enforce temporal smoothness directly on vertex positions:
\begin{equation}
    L_{\text{vert}}
    = \|S_i - S_{i-1}\|_1.
\end{equation}
% \SZ{Dobbiamo anche aggiungere che i loss sono pesati. Potresti mettere i pesi di fronte ai loss in equation 2 e 3 e poi dire che li stimiamo sul set di validazione.}
\mypar{Implementation details} We use an Adam optimizer for 300 epochs with early stopping. All our experiments run on a machine equipped with an A6000 GPU. In wall-clock time, it takes around \FP{Appena posso lancio una run per controllarlo più precisamente, dovrebbe metterci intorno ai 5 secondi per frame} around 5 seconds per frame. 


% ---------------------------------------------------------------
\subsection{Benchmark for the reconstruction of Animals from Monocular Videos}
\label{sec:dataset}

A substantial challenge of our task is the lack of datasets with
ground-truth 3D annotations, especially for the world coordinates.
To fill this gap, we introduce a new synthetic yet realistic benchmark with known 3D
geometry and camera parameters. 
We build on DeformingThings4D~\cite{DeformingThings}, which provides a large collection
of 4D mesh animations.
We first filter the sequences to retain only those that are realistic, discarding
atypical animals (\eg, dragons), physically implausible poses (\eg, swimming on
land), or too short (\ie, below one second).
Since the original textures have not been released, we retexture each mesh with
EmbodyGen~\cite{EmbodyGen}, which takes a mesh and a text prompt as input and
synthesises a plausible texture.
Each sequence is then rendered in a synthetic outdoor scene consisting of a flat ground
plane and an HDRI background, under three camera configurations designed to probe
different challenges: \emph{follow} (camera tracks the animal); \emph{fixed} (camera is fixed after the first frame); \emph{orbit} (camera rotates around the scene).
The first two configurations additionally receive a small random Gaussian jitter.
Camera azimuth, elevation, initial position, and distance are sampled randomly.
Further details are provided in the Supplementary Material.
Our Benchmark is composed by \RM{aggiungerei numeri una volta che le abbiamo}


% \begin{table*}[t]
% \tiny
% \centering
% \caption{Summary of notation used throughout the paper.}
% \label{tab:notation}
% \setlength{\tabcolsep}{6pt}
% \renewcommand{\arraystretch}{1.25}
% \begin{tabular}{@{}llll@{}}
% \toprule
% \textbf{Symbol} & \textbf{\LaTeX{} command} & \textbf{Description} & \textbf{Dimensionality} \\
% \midrule
% $S(\shape,\pose,\trasl,\grot)$ & \texttt{S(\textbackslash shape,\textbackslash pose,\textbackslash trasl,\textbackslash grot)}
%     & SMAL template mesh
%     & $\mathbb{R}^{V \times 3}$ ($V$ vertices) \\

% $\mathbf{F}$ & \texttt{\textbackslash mathbf\{F\}}
%     & Input RGB video
%     & $\mathbb{R}^{H \times W \times 3 \times N}$ \\

% $\image{i}$ & \texttt{\textbackslash image\{i\}}
%     & $i$-th RGB video frame
%     & $\mathbb{R}^{H \times W \times 3}$ \\

% $H,\,W$ & \texttt{H}, \texttt{W}
%     & Frame height and width (pixels)
%     & Scalars, $\mathbb{Z}_{>0}$ \\

% $N$ & \texttt{N}
%     & Number of frames
%     & Scalar, $\mathbb{Z}_{>0}$ \\

% $\pi(\,\cdot \mid C)$ & \texttt{\textbackslash pi(\textbackslash cdot \textbackslash mid C)}
%     & Differentiable renderer; maps a mesh to a 2D image under camera $C$
%     & Function: $\mathbb{R}^{V\times 3} \to \mathbb{R}^{H\times W}$ \\

% $C_i$ & \texttt{C\_i}
%     & Camera model for frame $i$ (intrinsics + extrinsics), from MegaSAM
%     & $\mathbb{R}^{3\times 4}$ \\

% $I_C^{\mathcal{M}}$ & \texttt{I\_C\^{}\{\textbackslash mathcal\{M\}\}}
%     & Rendered image of mesh $\mathcal{M}$ under camera $C$
%     & $\mathbb{R}^{H\times W}$ \\

% $\shape$ & \texttt{\textbackslash shape}
%     & SMAL shape (morphology) coefficients
%     & $\mathbb{R}^{|\shape|}$ (typically 10--20) \\

% $\pose$ & \texttt{\textbackslash pose}
%     & SMAL joint pose parameters (per-joint axis-angle)
%     & $\mathbb{R}^{3K}$, $K$ joints \\

% $\trasl$ & \texttt{\textbackslash trasl}
%     & Global translation of the animal in world space
%     & $\mathbb{R}^{3}$ \\

% $\grot$ & \texttt{\textbackslash grot}
%     & Global root rotation of the animal (axis-angle)
%     & $\mathbb{R}^{3}$ \\

% $M(\image{i})$ & \texttt{M(\textbackslash image\{i\})}
%     & Binary foreground mask from SAM for frame $i$
%     & $\{0,1\}^{H\times W}$ \\

% $\mathcal{B}(\,\cdot\,)$ & \texttt{\textbackslash mathcal\{B\}(\textbackslash cdot)}
%     & Soft boundary map of its argument; pixel values in $[0,1]$
%     & $[0,1]^{H \times W}$ \\

% $\partial(\cdot)$ & \texttt{\textbackslash partial(\textbackslash cdot)}
%     & Boundary / contour extraction operator
%     & Set of pixel coordinates \\

% $\mathcal{L}(\cdot)$ & \texttt{\textbackslash mathcal\{L\}(\textbackslash cdot)}
%     & Arc-length of a discrete contour
%     & Scalar, $\mathbb{R}_{\geq 0}$ \\

% $D(\,\cdot\,)$ & \texttt{D(\textbackslash cdot)}
%     & Depth map (rendered buffer or MegaSAM estimate)
%     & $\mathbb{R}^{H\times W}$ \\

% $\hat{S}$ & \texttt{\textbackslash hat\{S\}}
%     & SMAL template decorated with baked per-vertex DINO features
%     & $\mathbb{R}^{V\times d}$ \\

% $\Phi_v$ & \texttt{\textbackslash Phi\_v}
%     & DINO feature map rendered from view $v$ of Hunyuan3D mesh
%     & $\mathbb{R}^{H'\times W'\times d}$ \\

% $\mathbf{f}_u$ & \texttt{\textbackslash mathbf\{f\}\_u}
%     & Aggregated DINO feature vector at vertex $u$ of $\hat{S}$
%     & $\mathbb{R}^{d}$ \\

% $\mathcal{V}(u)$ & \texttt{\textbackslash mathcal\{V\}(u)}
%     & Set of views in which vertex $u$ is visible
%     & Subset of $\{1,\dots,V\}$ \\

% $\Pi_i$ & \texttt{\textbackslash Pi\_i}
%     & Rendered DINO feature map of $\hat{S}$ under camera $C_i$
%     & $\mathbb{R}^{H'\times W'\times d}$ \\

% $\tilde{F}_i$ & \texttt{\textbackslash tilde\{F\}\_i}
%     & DINO feature map extracted from video frame $\image{i}$
%     & $\mathbb{R}^{H'\times W'\times d}$ \\

% $d$ & \texttt{d}
%     & DINO feature dimensionality
%     & Scalar, $\mathbb{Z}_{>0}$ \\

% $\mathcal{P}_i$ & \texttt{\textbackslash mathcal\{P\}\_i}
%     & Set of valid (foreground) pixel indices in frame $i$
%     & Subset of $\{1,\dots,H'W'\}$ \\

% $\sigma_j$ & \texttt{\textbackslash sigma\_j}
%     & correspondence from rendered pixel $j$
%       to target pixel index
%     & Scalar index $\in \mathcal{P}_i$ \\

% $\pose_i,\,\pose_{i-1}$ & \texttt{\textbackslash pose\_i}, \texttt{\textbackslash pose\_\{i-1\}}
%     & Pose parameters at frames $i$ and $i{-}1$
%     & $\mathbb{R}^{3K}$ each \\

% $S_i,\,S_{i-1}$ & \texttt{S\_i}, \texttt{S\_\{i-1\}}
%     & Mesh vertex positions at frames $i$ and $i{-}1$
%     & $\mathbb{R}^{V\times 3}$ each \\
% \bottomrule
% \end{tabular}
% \end{table*}

==> sections/supmat/01_tech_det.tex <==

\begin{table}[b!]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{lcccccc}
\toprule
Stage & SAM & MegaSAM & Hunyuan3D & RSE & AniMer & Optimization \\
\midrule
Preprocessing & 10 s & 60 s & -- & -- & -- & -- \\
Initialization & -- & -- & 90 s & 30 s & 10 s & -- \\
Optimization & -- & -- & -- & -- & -- & 2000 s \\
\bottomrule
\end{tabular}
\caption{Runtime breakdown of the main stages of the pipeline for a case with $\sim$ 200 frames. Preprocessing includes mask extraction, initialization includes first-frame reconstruction and auxiliary setup, and optimization reports the runtime for 300 steps.}
\label{tab:runtime_breakdown}
\end{table}


\subsection{Implementation Details}
For all experiments, input frames are resized so that the maximum image dimension (width or height) does not exceed a fixed resolution. For real-world videos we use a maximum dimension of 512 pixels, while for the ORMA dataset and COP3D \cite{sinha2022common} we use 256 pixels. The higher resolution improves silhouette quality and geometric detail in real-world sequences, while the upper bound of 512 pixels is imposed by the AnyUP~\cite{wimmer2025anyup} model, which cannot process larger image resolutions.
\vspace{0.4cm}\\
Optimization runs for up to 300 iterations with early stopping, using a best-loss threshold of $10^{-4}$ and a patience of 100 iterations. After AniMer \cite{lyu2025animer} prediction over the video, we perform per-frame optimization to obtain the final reconstruction.
\vspace{0.4cm}\\
A detailed runtime breakdown of each pipeline stage is reported in Table \ref{tab:runtime_breakdown}. For a 200-frame sequence, the overall processing time is approximately 32 minutes and 50 seconds, compared to roughly 4.5 hours required by Animal Avatar.




\subsection{SMAL Registration}
\label{sec:smal_registration}
To register the SMAL model to the 3D point cloud obtained with Hunyuan3D we follow the approach described in \cite{Zuffi:CVPR:2017}, Equation 9. Specifically, we minimize an energy 
composed by a pose prior, a shape prior, and data terms of scan-to-mesh and mesh-to-scan distances.
Differently from \cite{Zuffi:CVPR:2017}, our pose prior is a simple L1 distance from an initial pose obtained with AniMer, and we do not use keypoints to guide the alignment. After aligning the SMAL model, we perform a model-free alignment of the vertices to the point cloud by optimizing over the SMAL model vertices under an As-Rigid-As-Possible regularization (see Equation 8 in \cite{Zuffi:CVPR:2017}). 


\subsection{Robust Semantic Correspondence}

Our robust semantic correspondences are derived from the textured Hunyuan3D reconstruction, whose texture provides stable visual cues for matching. We render a set of canonical views of the reconstructed mesh and extract dense DINO features from each view. Because these features capture fine-scale appearance details, such as fur patterns and local markings, they provide reliable cues for animal correspondence.
\begin{wrapfigure}[16]{r}{0.5\linewidth}
\scriptsize
\vspace{-1.2cm}
  \begin{overpic}[trim=0cm 0cm 0cm 0.0cm,clip, width=\linewidth]{figures/RSE.png}
	\end{overpic}
\captionof{figure}{We aggregate the DINO features from multiple views on the 3D shape surface. Such features are then used to establish a correspondence between the 3D shape and the video frames.}
 \vspace{-0.2cm} 
 \label{fig:DINO}
\end{wrapfigure}
These features are then projected back onto the reconstructed surface to obtain per-vertex descriptors, which are subsequently transferred to the SMAL model. In \cref{fig:DINO} we depict a visualization of feature aggregation on the animal's 3D surface. This produces a dense semantic representation on the SMAL surface, guiding the optimization toward semantically meaningful alignments. Additional details are provided in Sec.~4.1 of the main paper. 
% \begin{wrapfigure}
% \end{wrapfigure}
% \begin{figure*}[h!]
% \centering
% \begin{minipage}[t]{0.48\textwidth}
% \vspace{0pt}
% Our robust semantic correspondences are derived from the textured Hunyuan3D reconstruction, whose texture provides stable visual cues for matching. We render a set of canonical views of the reconstructed mesh and extract dense DINO features from each view. Because these features capture fine-scale appearance details, such as fur patterns and local markings, they provide reliable cues for animal correspondence.
% \vspace{0.5em}\\
% These features are then projected back onto the reconstructed surface to obtain per-vertex descriptors, which are subsequently transferred to the SMAL model. This produces a dense semantic representation on the SMAL surface, guiding the optimization toward semantically meaningful alignments. Additional details are provided in Sec.~4.1 of the main paper.
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.48\textwidth}
% \vspace{0pt}
% \centering
% \includegraphics[width=\linewidth]{figures/RSE.png}
% \caption{TBD.}
% \label{fig:semantic_correspondence}
% \end{minipage}
% \vspace{0.5em}\\
% \begin{minipage}[t]{0.98\textwidth}
Compared to CSE-based correspondences \cite{kulkarni2019csm}, this representation is substantially more stable over time. In practice, CSE predictions often vary across frames even under limited motion, whereas DINO-based features remain much more consistent, especially in articulated or visually distinctive regions. As shown in Fig.~\ref{fig:CSE}, this improved temporal stability leads to more reliable correspondences and reduces optimization drift.
% \end{minipage}
% \end{figure*}

\label{sec:rse}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/CSEvsDINO.png}
    \caption{Comparison between CSE features (top) and our DINO-based features (bottom). Note how the CSE features vary across visually similar frames.}
    \label{fig:CSE}
\end{figure}


==> sections/supmat/02_orma_dataset.tex <==

A major challenge for evaluating animal reconstruction methods is the lack of datasets with reliable 3D ground-truth annotations in world coordinates. Existing datasets such as COP3D\cite{sinha2022common} contain videos of real animals but do not provide ground-truth geometry or camera calibration, making it difficult to quantitatively verify whether reconstructed motion is correct in global space or to measure errors such as scale drift and temporally inconsistent poses.
\vspace{0.4cm}\\
To enable controlled evaluation, we generate a synthetic benchmark with full geometric supervision. Our dataset is built from \textit{DeformingThings4D}~\cite{li20214dcomplete}, which contains animated meshes represented as sequences of per-vertex deformation offsets applied to a canonical base mesh. Applying these offsets sequentially reconstructs the mesh animation describing the animal motion. The original dataset contains 1,972 deformation sequences across 26 categories.
Following the filtering procedure described in the main paper, we discard sequences that are unsuitable for terrestrial outdoor scenes, including aquatic animals, physically implausible motions, or sequences shorter than one second. After filtering, 121 candidate animations remain.
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/textures.png}
    \caption{Examples of generated textures.}
    \label{fig:textures}
\end{figure}
Because the original textures were not released, we generate new textures using \textit{EmbodyGen}~\cite{wang2025embodiedgengenerative3dworld}, which synthesizes plausible textures conditioned on a mesh and a text prompt. Multiple texture variations are generated for each animal category to increase appearance diversity (Fig. \ref{fig:textures}).
\vspace{0.4cm}\\
All sequences are rendered in a synthetic outdoor scene consisting of grassy terrain and HDRI sky illumination (note that, to ensure that the terrain provides realistic cues for depth and camera estimation, we use a 3D terrain asset rendered under the scene camera). For each animation we render three camera configurations: \emph{follow} (camera tracks the animal), \emph{fixed} (camera remains static), and \emph{orbit} (camera rotates around the scene). Camera azimuth, elevation, distance, and initial position are randomly sampled, and the follow and fixed configurations additionally include small Gaussian camera jitter.
\vspace{0.4cm}\\
For every frame we export RGB images, segmentation masks, depth maps, and the ground-truth mesh in world coordinates, together with the full camera calibration parameters (intrinsics and camera-to-world transformations).


\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{6}{c}{Species} &  \\
\cmidrule(lr){2-7}
Asset & Dog & Fox & Puma & Bear & Bucks & Husky & Total \\
\midrule
Animations & 51 & 47 & 16 & 4 & 1 & 1 & \textbf{121} \\
Textures   & 13 & 2 & 3 & 1 & 1 & 1 & \textbf{21} \\
\bottomrule
\end{tabular}
\caption{Statistics of the animal assets used in our synthetic dataset, including the number of animation sequences and generated texture variants.}
\end{table}

==> sections/supmat/03_more_results.tex <==
In this section we present additional qualitative results that complement the experiments reported in the main paper. These examples include further comparisons with concurrent methods, additional animal categories, limitations, and results on real video sequences from the COP3D \cite{sinha2022common} and Pferd \cite{Li2024PFERD} datasets.

To facilitate navigation through the supplementary material, we organize the results as follows:

\begin{itemize}
\item Method comparisons: pages 6--12
\item Additional animal categories: pages 13--16
\item Real-world videos (COP-3D and Pferd): pages 17--26
\end{itemize}

Each page contains several representative examples illustrating the robustness of our approach across different animal species, poses, and video conditions.

\subsection{Limitations and Failure Cases}
Our approach is subject to several limitations arising from the underlying model assumptions and the reconstruction pipeline.
\vspace{0.4cm}\\
First, some errors originate from limitations in the SMAL fitting process when representing certain pose variations present in real animals. Although the SMAL model is capable of representing ear articulation and mouth opening, in practice these degrees of freedom are often not properly recovered during optimization. Instead of activating the corresponding articulations, the optimizer may compensate by fitting the ears inside the silhouette or by positioning the mouth in regions where the silhouette is wider, sometimes leaving the jaw contour mismatched. Similarly, the model struggles to accurately represent seated poses, where the animal’s limbs and body undergo strong articulation and contact with the ground. Finally, errors may arise during the alignment between SMAL and Hunyuan3D meshes. When the two geometries differ significantly, the registration step can become unstable and produce an inaccurate final shape.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/Failurecases.png}
    \caption{Examples of failure cases. Left: errors in the SMAL fitting process when the animal opens its mouth. Although SMAL can represent mouth articulation, the optimization sometimes fails to recover it, leading to incorrect silhouette alignment. Right: Hun3D mesh registration failure caused by significant geometric differences between the meshes.}
    \label{fig:fail}
\end{figure}

\newpage
\subsection{More Comparisons}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/comp1.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/comp2.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/comp3.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/comp4.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/comp5.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/comp6.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/comp7.png}
\end{figure}
\subsection{Other Animals}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/oa1.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/oa2.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/oa3.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/oa4.png}
\end{figure}

\subsection{COP3D Results}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/cop1.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/cop2.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/cop3.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/cop4.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/results/cop5.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/results/cop6.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/results/cop7.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/results/cop8.png}
\end{figure}

\subsection{PFERD Results}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/PFERD1.png}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/results/PFERD2.png}
\end{figure}

